The time evolution of the ultraviolet habitable zone

For stars hosting Circumstellar Habitable Zone (CHZ) exoplanets, we investigate the time-evolution of their ultraviolet habitable zone (UHZ), the annular region around a star where an exoplanet could experience a suitable ultraviolet environment for the presence and emergence of life, and the possible intersection of the UHZ with the CHZ. To estimate their UV luminosity evolution, and therefore the evolution of their UHZ, we analyse Swift-UV/Optical telescope observations and adopt the near-UV luminosity evolutionary tracks derived using GALEX observations of young moving groups. We find that an intersection between CHZ and UHZ could exist (or have existed) around all stars of our sample at different epochs, except for the coldest M-dwarfs (temperature < 2800 K, e.g. Trappist-1). For hotter M-dwarfs the formation of RNA precursors through cyanosulfidic chemistry triggered by near-UV radiation could occur during the first 1-2 Gyrs. The radial-extension and time-duration of the CHZ-UHZ intersection increase with the stellar effective temperature and the exoplanet atmospheric transmissivity at near-UV wavelengths. Within our sample, Proxima Centauri represents a golden target for the quest of life outside the Solar system because it experienced a long-lasting and more extended, compared to similar M-dwarfs, CHZ-UHZ intersection.

==> letter_referee.tex <==
Scientific Editor's Comments:

The referee requests that the revised version be submitted in single-column mode, in order to provide clearer line numbers for the review copy than is possible in two-column mode.

Reviewer's Comments:
R) The manuscript describes the extension of the 'ultraviolet habitable zone' to include considerations of the time evolution of stellar luminosity. My chief concern is that this feels like an incremental advance on previously published work, but may not go far enough to demonstrate novelty and robustness to uncertainty or updated parameters. Below I describe several high-level comments that I'd like to see addressed before the manuscript is published. Additional comments directed at specific locations in the text are listed below that, using the page (L1-6), line (1-60) and left or right (l or r) columns, i.e., L1-49-l refers to page L1, line 49, left column. Ultimately, it's unclear how the results would change if the uncertainties in stellar ages and UV evolution are propagated through the model, but I expect that that is a necessary step in order to avoid obscuring the larger picture.

A) We thank the reviewer for the comments for our manuscript, which gave us the opportunity to greatly improve it. We respond to the reviewer's comments below. All changes in the revised manuscript are in bold. We agree with the referee regarding the necessity to consider uncertainties in stellar ages. In this revised version we show how these uncertainties influence the results. Our previous work regarding the ultraviolet habitable zone "The ultraviolet habitable zone of exoplanets" (Spinelli, R., Borsa, F., Ghirlanda, G., et al. 2023, MNRAS, 522, 1411) conclude that all the exoplanets discovered in the classical habitable zone around M-dwarfs currently does not received the NUV flux required for the prebiotic chemistry described in Rimmer et al. 2018. Generalizing this argument leads to the conclusion that M--dwarfs, the most abundant stellar population (~70\%) in the Galaxy, may not be sufficiently NUV luminous to trigger the origin of life according to this specific prebiotic pathway (Buccino et al. 2007, Rimmer et al. 2018, Ranjan et al. 2017). This submitted work overturns this perspective, arguing that considering the NUV luminosity evolution of the M dwarfs, most of them could irradiate the habitable zone exoplanets with NUV flux suitable for the prebiotic chemistry described in Rimmer et al. 2018 during the first 1-2 Gyrs of their evolution. This suggest that the conditions for the origin of life according to these prebiotic pathways may be or may have been common in the universe. Therefore we believe that this work represent a significant advancement of knowledge regarding the habitability of exoplanets.

R) Major comments: - The GALEX dataset (Richey-Yowell et al., 2023) that describes a large population of stars, and even when dividing them into narrower stellar mass ranges, the variability in fluxes span 1-3 orders of magnitude. Part of this variability could be due to the assumption that the stars not in the young moving groups are given a fixed age of 5 Gyr, although that some bimodality is seen in the NUV and X-ray flux density distributions (Figs. 3 and 8). Additionally, the GALEX photometry (ibid.) and Swift UV grism (Chavali et al., 2022) are not compatible with the stated NUV band used by Rimmer et al. (2018). GALEX reports the NUV (177-283 nm) and FUV (134-179 nm) and the UV grism of Swift covers 170-290 nm, as compared to the 200-280 nm region determined by Rimmer et al. (2018). For earlier stars this is less of an issue, since the UV drops off towards shorter wavelengths, but later stars are essentially flat across this wavelength region. This implies that taking the GALEX observations as a stand-in for the wavelength of interest is a conservative estimate of the NUV flux of later stars.

A) We agree with the referee regarding the limitations of the GALEX dataset assumption that stars not in the young moving groups are given a fixed age of 5 Gyr (assuming  5 Gyr at the average age of the field stars nearby to our Sun). However, this is a well-known problem in the literature, for which a clear solution to establish age for stars older than $\sim$500 Myr and not in the young moving groups has not yet been found. We declare this assumption in the text but a solution of this problem is beyond the scope of this article and requires a method that derives the stellar age of the GALEX sample. Nevertheless in this revised version, we estimate the uncertainties on the results derived taking into account the uncertainties on the stellar ages (see following answers). Regarding the compatibility between GALEX photometry and Swift UV grism in this revised version we use the following approach. As suggested by Richey-Yowell et al., 2023 (equation A1), we convert the GALEX flux density in Jansky to the flux density in erg cm$^-2$ s$^-1$ A$^-1$ using the mean effective NUV wavelengths derived by Schneider \& Shkolnik (2018) for M dwarfs (2553 Angstrom) and Richey-Yowell et al., 2023 for K stars (2623 Angstrom) which take into account the spectral shape of M and K stars in the total GALEX bandwidth (177-283 nm). Then we assume this flux density as the mean of the flux density in the 200-280 nm and we obtain an estimation of the integrated flux in this bandwidth by multiplying this mean flux density for 800 Angstrom (the bandwidth considered by Rimmer et al. 2018). This assumption is supported by visual inspection of archival NUV data obtained by HST/STIS and spectra delivered by the treasury MUSCLES survey (France et al. 2016, see for example the HST-STIS-230 spectra of the M-dwarfs GJ 1132, GJ163, GJ 436 and K stars WASP-43 and HAT-P-26 at https://archive.stsci.edu/prepds/muscles/). For Swift observations, we convert the count rate to flux density in erg cm$^-2$ s$^-1$ A$^-1$ using the conversion factor derived by Brown et al. 2016 and then we multiply this value to 800 to obtain an estimation of the flux in the 200-280 nm band. 

R) The uncertainties in stellar ages are not addressed. The manuscript uses the stated ages of the host stars where possible and then bounds the UV emissions of the stars with only lower limits on their age between that value and the age of the universe.

A) In this revised version we addressed the uncertainties in stellar ages. We report the error on the age in Table 1. To obtain an error on the time of overlap between the optimistic habitable zone and the ultraviolet habitable zone we estimate the NUV evolutionary track for each target using the measured NUV luminosity and the upper and the lower age. We repeat the procedure for these 3 values of the age. This gives the central value and the error reported in Figure 3 and Figure 4. We add a paragraph in the main text to explain how we consider these uncertainties and we update the figures 3 and 4 that shows results with the errors.  

R) Planetary evolution is important here, since the formation of prebiotic materials on a Venus-like planet will likely not preserve those materials into a more clement period. I'd suggest that a consideration of the continuously habitable zone is more relevant to late M dwarfs, particularly in light of their protracted pre-main sequence luminosities.

A) We agree with the referee regarding the importance of planetary evolution. Although a detailed description of this is beyond the scope of our work, we use the New Planetary Synthesis Model to explore planetary evolution. We answer about this point in the following answer. If we consider the continuously habitable zone also in the pre-main sequence phase, the overlap between the UHZ and the continuously habitable zone is higher at each time of the evolution. Although at the beginning of the stellar evolution, the continuously habitable zone was too hot to stably host liquid water over a large fraction of their surfaces, the building blocks of life could have been accumulated very rapidly compared to geological time scales, in a local transient environment, for which liquid water could be present outside the liquid water habitable zone (see also Rimmer et al. 2018). For this reason, assuming the evolving habitable zone (not continuously) is a conservative choice. 

R)The phrasing 'evolve backward in time' is not correct and doesn't capture the work described in the remainder of the text. The methodology scales the UV flux with time given the observed stellar parameters and age of the star at the present day.

A) We reviewed this phrase in the text.

R) Line-specific comments: L1-48-l - as I understand it, all of the known rocky planets in their host stars' habitable zones are orbiting M dwarfs.

A) The great majority but not all planets orbiting in the optimistic habitable zone are around M-dwarfs. Examples around K-stars are: Kepler-62 f, Kepler-62 e, HD 40307 g, Kepler-442 b, Kepler-1410 b (see the complete list on https://phl.upr.edu/hwc). Kepler-452 b, Kepler-1638 b, Kepler-22 b and Kepler 1606 b orbiting around G-stars. We selected all rocky planets in the optimistic habitable zone with Swift UVOT observations. 

R) L1-51-l - Not clear why LAWKI abbreviation is needed, as the phrase is used here and on the next page.

A) We eliminate this abbreviation. 

R) L1-39-r - The Zsom et al. (2013) reference unphysically controls relative humidity to drive changes to the inner edge of the habitable zone, in direct conflict with the assumptions that underpin the conventional habitable zone (e.g., stable liquid water on the surface). A more pertinent discussion in the literature is Goldblatt et al. (2013) and Ramirez et al. (2014) for CO2-driven runaway greenhouses, or the more recent 3-D exploration by Chaverot et al. (2023) that includes some variability in the transition based on atmospheric composition.

A) We thank the referee for pointing out this limitation of Zsom et al. (2013) and for suggesting other interesting articles on the topic. We have updated these references taking these comments into account.

R) L1-47-52-r - This sentence is incomplete ("...may cause atmospheric evaporation and (Sanz-Forcada..., biomolecules destruction.")

A) We reviewed this phrase in the text.

R) L1-55-r - this sentence is a phrased awkwardly. Would suggest "...UV light is crucial for the synthesis of some of the building blocks of life, up to and including ribonucleic acid (RNA)." One could argue that UV light is a prerequisite for all photochemistry, making some parts of the sentence redundant.

A) We reviewed this phrase in the text following the suggestion of the referee.

R) L2-13-l - "...composed [of] old stars..."

A) We reviewed this phrase in the text.

R) L2-8-9-r - see first comment about ages.

A) As we answer before, in this revised version we addressed the uncertainties in stellar ages. 

R) L2-22-r - It's not clear that a linear interpolation between NUV evolutionary tracks is the best approach. Other isochrone datasets (e.g., Baraffe et al., 2015; Hidalgo et al., 2018) use a linear interpolation in terms of mass, but parameterizations of UV fluxes scale them with bolometric luminosity (e.g., Sanz-Forcada et al., 2011; Peacock et al., 2020). Bolometric luminosity is only linear with stellar mass for very high-mass stars, and is generally second- to fourth-order (e.g., Maurizio and Cassisi, 2005).

A) Isochrone datasets do not provide the NUV luminosity at each time of the evolution of a star. Our approach is similar to that used in literature for the X-ray and the EUV stellar emission. For example, based on X-ray observations of young open clusters, Penz et al. 2008 and Penz \& Micela 2008 construct a scaling law for X-ray emission of G and M-stars for ages between 0.1 and 10 Gyr. Then, Sanz-Forcada et al. 2011 and 2022 found a scaling law between X-ray and EUV emission. To model the X-ray and the EUV luminosity evolution of a star with observations in these bands today, many works assumed this scaling relation anchored to the X-ray value measured today. We used this same approach using the Near UV luminosity measured by the Swift Telescope and using the scaling law obtained using NUV GALEX observations on young moving groups.

R) L2-24-25-r - no errors are included when considering the current ages of the host stars. For example, Bazot et al. (2016) is a theory paper that reports uncertainties of ~1 Gyr in Proxima Centauri's age, but Beech et al. (2017) suggest that an age of 7-8 Gyr is more consistent with observations. Additionally, the reported age for K2-18 (2.4 Gyr) points to an older Guinan and Engle reference (2019), whereas Engle and Guinan (2023) reports an age of ~3.35+-0.45 Gyr, suggesting that the age values are not fully up-to-date and considering uncertainties is a necessary step in discussing this topic. This compounds the original broad binning of age-less stars to 5 Gyr done by Richey-Yowell et al. (2023).

A) In this revised version we addressed the uncertainties in stellar ages. We report the error on the age in Table 1 from the same references of the current ages. In this revised version we assume for Proxima Centauri and K2-18 the most updated ages suggested by the referee. In the discussion, we report how the results change if we assume different age estimations for Proxima Centauri.  

R) L2-41-42-r - what does transmissivity of 100\%, 50\%, and 10\% correspond to in terms of composition or pressure? Where do such atmospheres appear in the solar system or Earth's history? These are otherwise divorced from the practical side of planetary evolution.

A) In this work we assume NUV transmissivity as a free parameter. For our purpose, we refer to a planet with 50\% of NUV transmissivity as a planet with an atmosphere with a pressure and a composition such as allows half of the radiation incident above the atmosphere to reach the surface of the planet. The choice to treat NUV transmissivity as a free parameter is based on the consideration that also for early-Earth we are poor constraints about this factor, since the NUV transmissivity in the band of interest in our work (200-280 nm) strongly depends on the 03 and CO2 concentrations (see Figure 4 in Cockell et al. 2007). 
For example, for the Earth's history, we could assume as a reference Cockell et al. 2001 (The History of the UV radiation Climate on the Earth - Theoretical and Space-based Observations) and Cockell et al. 2007 (Habitat of early life: Solar X-ray and UV radiation at Earth's surface 4-3.5 billion years ago). In this latter work, the authors calculated the atmospheric extinction for radiation between 0.1-320 nm, assuming different atmospheric compositions for the Archean Earth (between 4 and 3 Gyr, when life formed on Earth). We considered these 3 different Archean atmospheric composition models as suggested by Kasting et al. 1993 and Canuto et al. 1982 (see Table 1, Table 2, and Figure 5 in Cockell et al. 2007) with different C02 compositions: 2.62e19 cm-3 (surface pressure 1 bar), 5.24x10e18 cm-3 (0.8 bar) and 5.24x10e17 cm-3 (0.8 bar). We integrated in the 200-280 nm band the flux at the top of the atmosphere of the Archean Earth and the surface irradiation assuming these 3 different atmospheres (Figure 5 in Cockell et al. 2007). The ratio between this two flux give us an estimation of the atmospheric NUV transmissivity for the Earth Archean period that is 70\%-20\%-1\% for different models. This demonstrates how this value is sensitive to the unknown C02 composition. After the Archean, the Great Oxidation Event in the Early Proterozoic (2 Gyr ago) led to the increase of oxygen in the atmosphere, drastically reducing the NUV transmissivity to 0\% (the same value of today). As mentioned in the discussion, modeling the evolution of the atmospheric composition of a given planet is beyond the scope of this work. Neverthless, a change (on a geological time scale) in the NUV transmission of the atmosphere can be visualized in our plots by switching between region of different colors (bottom panels in Fig. 2) during the evolution of the system. 

R) L2-51-51-r - The description of the colors appears to be repeated.

A) We eliminated the description of the colors in Figure 2. 

R) L3-1-r - The age of the universe as an upper bound may be unrealistic and feeds into my prior comment about including age uncertainties to communicate more information about how this prescription impacts the results.

A) As suggested by the referee, in this revised version we assume a more conservative upper limit (the age of the Milky Way 11 Gyr). 

R) L4-Fig 2 - I'd recommend a vertical line to denote a set of lines bounding the estimated time to form a rocky planet. Primordial atmospheres are often incredibly thick and this would likely push some of the targets to be more conservatively evaluated.

A) The time for a planet to entirely evaporate the primordial atmospheres and to become a naked rocky planet (with possibly a second atmosphere) depends on many factors such as the XUV luminosity of the star, the core of the planet, and the initial atmospheric mass fraction of primordial atmospheres. To add vertical lines as requested by the referee that indicate the time to form a rocky planet without a hydrogen and helium envelope we used the following approach. We exploited The New Generation Planetary Population Synthesis (NGPPS, Burn et al. 2021) simulations for low mass stars. This planetary formation model includes planetary migration, N-body interactions between embryos, accretion of planetesimals and gas, and the long-term contraction and loss of the gaseous atmospheres. We downloaded the following simulations at different time-step thanks to the permission of the Data and Analysis Center for Exoplanets group (DACE,University of Geneva): 
- NGM11New Generation Planetary Population Synthesis. Nominal model. 50 embryos per disk initially. 0.5 Msun stars. Burn et al. 2021.
- NGM10New Generation Planetary Population Synthesis. Nominal model. 50 embryos per disk initially. 0.1 Msun stars. Burn et al. 2021.
- NGM14New Generation Planetary Population Synthesis. Nominal model. 50 embryos per disk initially. 0.3 Msun stars. Burn et al. 2021.
- NGM12New Generation Planetary Population Synthesis. Nominal model. 50 embryos per disk initially. 0.7 Msun stars. Burn et al. 2021.

This simulation provides at each time-step of the planetary evolution from 1 Myr to 10 Gyr many planetary parameters (orbital distance, planetary mass, envelope mass, planetary radius etc...) for all the simulated planetary systems.

For each time-step we calculated the fraction of systems with at least one rocky planet (within the criteria of Spinelli et al. 2021) without a primordial envelope (envelope mass fraction equal to 0) in the continuously habitable zone. For all type of stars this fraction increases with time under the effect of photoevaporation. The slope of this growth is different for systems around stars with different masses and ends at different values at 10 Gyr (0.46 for 0.1 and 0.5 Msun, 0.42 for 0.7 Msun, 0.54 for 0.3 Msun). 

In the plots, we report with yellow, orange and dark orange lines the age at which this fraction is equal to 20\%, 30\%,  40\% for each system (Figure 2).

R) L5-24: Chavali et al. (2022) is an observation of one "young [early] M-dwarf" (not "M-dwarfs") and not sufficient to discount the long list of prior works.

A) We thank the referee for this suggestion. We reviewed this phrase in the text following the suggestion of the referee. 

R) L5-57-l - Why the mean value for only GJ 1061 and LHS 1140? This seems to suggest an age preference, as opposed to uncertainty.

A) In this revised version for this calculation we use both the value for the lower limit of the age provided by the literature and 11 Gyr (the age of the Milky Way). 


==> letter_referee_2.tex <==
Reviewer's Comments:
Reviewer: 1
Comments to the Author

We thank the reviewer for the minor comments for our manuscript, which gave us the opportunity to further improve it. We respond to the reviewer's comments below. All changes in the revised manuscript are in bold blue.

R) Our previous work regarding the ultraviolet habitable zone ...Spinelli et al....2023... conclude that all the exoplanets discovered in the classical habitable zone around M-dwarfs currently does not received the NUV flux required for the prebiotic chemistry described in Rimmer et al. 2018." This is not reflected in the conclusion, and I think it would make clear the novelty of this work if it did so.

A) We add a paragraph to clarify this point in the discussion. 

R) The response included a description of what the transmissivities were tied to, but that text does not appear in the manuscript. I'd like to see the transmissivities rooted to something physical for the reader.

A) We used the Earth’s archean atmospheric model cited by Cnossen et al. 2007 to calculate the CO2 concentrations that correspond to the transmissivities used in our work. We add a paragraph in sect. 4. 

R) Assuming an age of 4.8 Gyr for Proxima Centauri as suggested by Bazot et al. (2016)..." - it's not clear why this exceptional treatment is included for Prox Cen. If the authors prefer this value over that of Beech et al., or wish to perform additional analyses on all the age estimates for Prox Cen, then there should be an expanded discussion of why and what implications those uncertainties have. Otherwise, this feels like cherry-picking a reference to tell an optimistic story.

A) As suggested by the referee in the previous report, in this revised version we used the age estimated by Beech et al. 2017 because this work is more consistent with observations. In particular Beech et al. 2017 applied the Vogt-Russell theorem that suggested that once the mass and composition of a star are set, the equations of stellar structure must yield unique expressions for the radius, temperature and luminosity. Since these latter quantities and the mass are well constrained for Proxima Centauri, Beech et al. 2017 applied this theorem to derive the stellar metallicity. They found a lower metallicity with respect to the α Cen AB binary metallicity estimated in literature. This is inconsistent with an in situ or coevally origin with the α Cen AB binary (with an age of 5.0+-0.5 Gyr). Given the properties of Proxima Centauri, the value of its spin-period (83.5 days) and its relatively low flaring activity Beech et al. 2017 derived an age between 6-7 Gyr. We considered the approach relatively simple and convincing. 

Since we noticed a controversial debate in literature (e.g. Feng et al. 2018) regarding the age of Proxima Centauri (also concerning the true origin and the evolution of the triple system α Cen) and we found a unique level of intersection between UHZ and HZ for Proxima Centauri, we decided to explore if its high level of UHZ-HZ intersection respect to others M dwarfs change with the age value reported by Bazot et al. 2016. Their estimation lead to an average reduction of the the level of intersections by 25\% but it is still significantly higher than other M dwarfs (if we reduced the red point to 2.1 Gyr and the gray point to 1.0 Gyr for Proxima Centauri in Figure 4, this value is still significantly higher than the value obtained for other cold M dwarfs). We add a paragraph to explain these estimations for Proxima Centauri. 

R) Figure 2 - I'd bold the vertical lines. Also describe the gray shaded region around the gray line.

A) We bolded the vertical lines and we described the gray shaded region around the gray line in the caption. It represents the error on the estimated age of the planetary system. 

R) Figure 3 - I would label the sub-panels directly with information about transmissivity. Also the list of colors isn't tied to the overlap, it's tied to the transmissivity - potentially confusing for a reader.

A) We label the sub-panels.

R) This statement is also supported by the Swift NUV observations of a young M-dwarf (AU Mic) performed by Chavali et al. (2022)." It's a single star, so "M dwarf" is singular.

A) We corrected this sentence. 

R) Despite a detailed discussion of these issues is beyond the scope of this work, in Fig. 2)..." - I would rephrase as "A detailed discussion of these issues is beyond the scope of this work, but in Fig. 2...". Also note that there's a closing parenthesis that isn't matched here. Further, the colors are listed early in the paragraph, but not described until the end, potentially leading to confusion for the reader.

A) We corrected this sentence according to the referee's suggestion. 

R) To conclude we emphasize the case of Proxima Centauri b..." - but at present, Prox Cen isn't in the conventional habitable zone, and as such I'd like to see that reflected in the interpretation and outlook given here.

A) We did not fully understand the request of the referee. The misunderstanding might be because we are not clear on what the referee means by "conventional habitable zone." Proxima Centauri b orbits around its host star with a semi-major axis of 0.049 AU (Faria et al. 2022). This value is within the boundary limits that we assumed for the habitable zone (the optimistic habitable zone described by Kasting et al. 1993 and Kopparapu et al. 2014, Sect 2 of our work). According to our estimation, for Proxima Centauri, these limits are equal to 0.035 - 0.090 AU. Moreover, Proxima Centauri b is also within the conservative habitable zone defined by Kopparapu et al. 2013 (between Runaway Greenhouse and Maximum Greenhouse limits, 0.042-0.82 AU), as also reported by Meadows et al. 2018. For this reason, the Arecibo Catalogue (https://phl.upr.edu/hwc) puts Proxima Centauri b in the conservative sample of habitable zone exoplanets. 

